StraightLine: An End-to-End Resource-Aware Scheduler for Machine Learning Application Requests

The life cycle of machine learning (ML) applications consists of two stages: model development and model deployment. However, traditional ML systems (e.g., training-specific or inference-specific systems) focus on one particular stage or phase of the life cycle of ML applications. These systems often aim at optimizing model training or accelerating model inference, and they frequently assume homogeneous infrastructure, which may not always reflect real-world scenarios that include cloud data centers, local servers, containers, and serverless platforms. We present StraightLine, an end-to-end resource-aware scheduler that schedules the optimal resources (e.g., container, virtual machine, or serverless) for different ML application requests in a hybrid infrastructure. The key innovation is an empirical dynamic placing algorithm that intelligently places requests based on their unique characteristics (e.g., request frequency, input data size, and data distribution). In contrast to existing ML systems, StraightLine offers end-to-end resource-aware placement, thereby it can significantly reduce response time and failure rate for model deployment when facing different computing resources in the hybrid infrastructure.

==> 2_background.tex <==
\section{Related Work}
\label{sec:motivation}

\begin{comment}
\begin{figure}[t]
%\vspace{-0.1in}
 \centering
 %\vspace{-0.05in}
 \includegraphics[width=0.98\linewidth]{figures/3.1.2-MLApplicationLifeCycle-new.pdf}
  %\vspace{0.3in}
  %\vspace{-0.1in} 
 \caption{The conceptual life cycle of \ac{ML} applications. In model development, the streaming data serves as the training data and goes over a predefined data pipeline, and \ac{ML} models are trained and verified with processed data in the local infrastructure (e.g., in-house data center, local server, or docker containers). In model development, the trained \ac{ML} models are then deployed on the infrastructure composed of different computing resources. Then, applications services send requests to the infrastructure through, for example, RESTful APIs.}
 \label{fig:MLapplicationLefiCycle}
% \vspace{-0.05in} 
\end{figure}
\end{comment}

\begin{comment}
In this section, we first summarize the life cycle of \ac{ML} applications in §\ref{subsec: backgroud}, and then review existing \ac{ML} applications systems to understand the gap between development and deployment of ML applications in §\ref{subsec: review}.

\subsection{Background}
\label{subsec: backgroud}

Figure \ref{fig:MLapplicationLefiCycle} shows the life cycle of \ac{ML} applications. Model development and model deployment are two major stages.

\textbf{Model development}. 
It consists of the following three phases: (i) data management, (ii) model learning, and (iii) model verification \cite{ashmore2021assuring}. Data is an integral part of any \ac{ML} applications. The overall predictive performance of \ac{ML} applications largely depends on the training and test data as much as on the learning algorithms. The process of producing quality datasets is usually the very first stage in any production \ac{ML} pipeline.
Since data management and collection lack of a standard approach and measurement, it is assumed that the data management can implemented as data pipeline by big data generators, such as sensors, log collectors, and transaction data collectors. 
Model learning is the phase of model development that draws the most attention within the \ac{ML} community. Generally speaking, model is selected to be used to prove the concept of the proposed ML solution and get the end-to-end setup in place \cite{wagstaff2019enabling}. Then, the chosen model is fed with a collected dataset in order to learn certain patterns or representations of the data in the hybrid infrastructure of an in-house data center, local servers, or docker containers. 
Lastly, model verification is regarded as a fundamental step to ensure the quality of the product and reduces maintenance costs. ML models are expected to generalize well to unseen data, demonstrate reasonable performance on edge cases and overall robustness, as well as reach specified functional requirements \cite{paleyes2020challenges}.

%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
\center
 \includegraphics[width=1.\linewidth]{figures/1.1-OverAllDesign-4.pdf}
\caption{The workflow and three layers in {\systemNameAbbr}. In Layer 1, {\systemNameAbbr} uses NVIDIA-Docker to define the execution in model development. In Layer 2, {\systemNameAbbr} deploys multiple implementations for \ac{ML} applications. In Layer 3, {\systemNameAbbr} runs the online resource placement algorithm to place computing resources for upcoming \ac{ML} requests.}
\label{fig:3 layers}
% \vspace{-0.2in}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%

\textbf{Model deployment}. This stage consists of two major phases: (i) infrastructure building and (ii) model implementation. In real-world industrial environments, the infrastructure is hybrid, which includes in-house data centers, local servers, docker containers, serverless platforms (e.g., AWS Lambda \cite{AmazonLambda}), to provide lower inference latency and response time. Such a hybrid infrastructure offers a variety of \ac{ML} services and implementations in a collaborative fashion, whereas model implementation mainly focuses on how \ac{ML} applications are implemented and incorporated into the infrastructure to shorten latency or response time. Traditionally, a trained \ac{ML} model can serve as a RESTful API \cite{sohan2015spyrest} or a lightweight web server (e.g., Flask \cite{flask}). Moreover, enterprise-level solutions and open-source solutions, such as  Microsoft's ML.NET \cite{mlnet} and Deep Java Library \cite{DJL} are also available. For small or middle-size companies, the on-demand cloud computing ML platforms, such as AWS ML \cite{AWSML} and Azure ML REST API \cite{microsoftazure} are also suitable for \ac{ML} implementations. Recently, Docker containers \cite{anderson2015docker} and serverless computing \cite{baldini2017serverless} offer more portable options as \ac{ML} applications usually require different operating systems, ML application runtime (e.g., TensorFlow \cite{abadi2016tensorflow}, PyTorch \cite{NEURIPS2019_9015}, PyWren \cite{jonas2017occupy}, etc.), and language environment like Python, Java, or R. Docker containers and serverless computing offer plug-and-go computing services as they can connect target environments automatically.

\subsection{Related Work}
\label{subsec: review}
\end{comment}

Elshawi et al. presented a framework that includes the basic clouding computing resource (e.g., storage, CPU, and memory), data streaming platforms (e.g., Hadoop \cite{hadoop}, Spark \cite{zaharia2012resilient}, Flink \cite{carbone2015apache}) and workflow environment (e.g., Spark \cite{zaharia2012resilient}, Google ML \cite{googleml}, TensorFlow \cite{abadi2016tensorflow}, KeyStone ML \cite{keystoneml}). The proposed framework supports the \ac{ML} application workflow from data management to model training while it does not support ML application services \cite{ELSHAWI20181}. 

Wang et al. presented Rafiki, an \ac{ML} analytics service system to provide the training and inference service of \ac{ML} models. Howerver, Rafiki is limited to 3-node cluster, so it is not applicable to hybrid infrastructure \cite{wang2018rafiki}.

Sánchez-Artigas et al. proposed a Serverless enabled ML system, MLLess, which achieves 15 times faster than serverful ML applications and successfully reduces the cost. The paper compared the ML model training process in detail by using PyTorth and PyWren on local data centers and serverless environments respectively \cite{sanchez2021experience}. However, the experiment assumes that all the training environments use CPU clusters since the GPU cluster is not supported by Lambda. This generates a critical bias from the real-world applications as GPU cluster has become a fundamental requirement for ML applications.


Naranjo et al. proposed a serverless gateway for event-driven \ac{ML} inference in multiple clouds. This paper presented a framework that allows packaging the inference function as a RESTful API on both serverless and on-premises cloud \cite{naranjo2021serverless}. However, the paper focuses more on the feasibility of the proposed framework. The performance differences between on-premises and serverless resources are not discussed. The paper also focuses on the inference function based on a pre-trained model. The model development is overlooked even though an AWS Batch is included in the framework which can provide GPU cluster support for the model training.

Shukla et al. proposed an anomaly detection application for Internet-of-Things (IoT) devices over edge computing networks. The data is collected by IoT sensors and sent to the edge for model training and deployment. For model inference, IoT devices send data to edge for model inference and the edge sends the inference results to the cloud for analytics \cite{shukla2022novel}. However, the paper only focuses on a single edge-based environment while ignoring the hybrid infrastructure. 


%Most of works focus on one single stages or phases in the life cycle of \ac{ML} applications. Moreover, most of the work assumes that the infrastructure for \ac{ML} applications is unified and monotonous. This serves as the motivation of this paper to offer an end-to-end system for \ac{ML} applications.




